Double frame Tomographic PTV at high seeding densities

A novel method performing 3D PTV from double frame multi-camera images is introduced. Particle velocities are estimated by following three steps. Firstly, separate particle reconstructions with a sparsity-based algorithm are performed on a fine grid. Secondly, they are expanded on a coarser grid on which 3D correlation is performed, yielding a predictor displacement field that allows to efficiently match particles at the two time instants. As these particles are still located on a voxel grid, the third, final step achieves particle position refinement to their actual subvoxel position by a global optimization process, also accounting for their intensities. As it strongly leverages on principles from tomographic reconstruction, the technique is termed Double-Frame Tomo-PTV (DF-TPTV). Synthetic tests on a complex turbulent flow show that the method achieves high particle and vector detection efficiency, up to seeding densities of around 0.08 particles per pixel (ppp), while its root-mean-square error of velocity estimation is lower to that of state-of-the-art similar methods. Results from an experimental campaign on a transitional round air jet at Reynolds number 4600 are also presented. During the tests, seeding density varies from 0.06 to 0.03 ppp on average. Associated to an outlier rejection scheme based on temporal statistics, DF-TPTV vector fields truthfully correspond to the instantaneous jet dynamics. Quantitative performance assessment is provided by introducing statistics performed by bin averaging, upon assuming statistical axisymmetry of the jet. Mean and fluctuating axial velocity components in the jet near-field are compared with reference results obtained from planar PIV at higher seeding density.

==> alphabet.tex <==
% Document LaTeX	Auteur : Guy Le Besnerais	Date : 25/05/94
% Modification : J.-F. Gio	(15/09/95)
%			        J.I. (format Latex 2e, taille adaptative 22/03/99)

% Objet : Definitions compactes d'alphabets pour ecriture en Math
% b pour bold italique : \Ab
% v pour bold droit : \Av
% D pour droit : \AD
% Capitale pour capitale : \Lambda

\typeout{\space}
\typeout{\space\space\space\space Fichier 'alphabet.tex' -- LSS 1994/95/99}
\typeout{\space\space\space\space (necessite les packages xspace et amsmath)}
\typeout{\space}

\RequirePackage{amsmath}
\RequirePackage{xspace}

%%%% NEW - NEW - %%%%% Small caps gras %%%% 05-06-98 %%%% JFG %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%% Merci \`a Caro %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareFontShape{T1}{cmr}{bx}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}
% SC en bold (Hack !)
\DeclareFontShape{T1}{cmr}{b}{sc}{
	 <8> <9> <10> <10.95> dcbsc10
	 <12> <14.4> dcbsc10
	 <17.28> <20.74> <24.88> dcbsc10
	 }{}%

\def\scb#1{\bfseries {\scshape #1}}%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% DEFINITIONS PRELIMINAIRES 

% definition pour \xspace
\def\XS{\xspace}

% Style gras italique (Necessite amsmath)
\def\sbm#1{\ensuremath{\boldsymbol{#1}}}               

% Style droit en math
\def\sdm#1{\ensuremath{\mathrm{#1}}}

% Style gras droit
\def\sbv#1{\ensuremath{\mathbf{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ALPHABET GRAS ITALIQUE
% Taille adaptative

\def\Ab{{\sbm{A}}\XS}  \def\ab{{\sbm{a}}\XS}
\def\Bb{{\sbm{B}}\XS}  \def\bb{{\sbm{b}}\XS}
\def\Cb{{\sbm{C}}\XS}  \def\cb{{\sbm{c}}\XS}
\def\Db{{\sbm{D}}\XS}  \def\db{{\sbm{d}}\XS}
\def\Eb{{\sbm{E}}\XS}  \def\eb{{\sbm{e}}\XS}
\def\Fb{{\sbm{F}}\XS}  \def\fb{{\sbm{f}}\XS}
\def\Gb{{\sbm{G}}\XS}  \def\gb{{\sbm{g}}\XS}
\def\Hb{{\sbm{H}}\XS}  \def\hb{{\sbm{h}}\XS}
\def\Ib{{\sbm{I}}\XS}  \def\ib{{\sbm{i}}\XS}
\def\Jb{{\sbm{J}}\XS}  \def\jb{{\sbm{j}}\XS}
\def\Kb{{\sbm{K}}\XS}  \def\kb{{\sbm{k}}\XS}
\def\Lb{{\sbm{L}}\XS}  \def\lb{{\sbm{l}}\XS}
\def\Mb{{\sbm{M}}\XS}  \def\mb{{\sbm{m}}\XS}
\def\Nb{{\sbm{N}}\XS}  \def\nb{{\sbm{n}}\XS}
\def\Ob{{\sbm{O}}\XS}  \def\ob{{\sbm{o}}\XS}
\def\Pb{{\sbm{P}}\XS}  \def\pb{{\sbm{p}}\XS}
\def\Qb{{\sbm{Q}}\XS}  \def\qb{{\sbm{q}}\XS}
\def\Rb{{\sbm{R}}\XS}  \def\rb{{\sbm{r}}\XS}
\def\Sb{{\sbm{S}}\XS}  \def\sb{{\sbm{s}}\XS}
\def\Tb{{\sbm{T}}\XS}  \def\tb{{\sbm{t}}\XS}
\def\Ub{{\sbm{U}}\XS}  \def\ub{{\sbm{u}}\XS}
\def\Vb{{\sbm{V}}\XS}  \def\vb{{\sbm{v}}\XS}
\def\Wb{{\sbm{W}}\XS}  \def\wb{{\sbm{w}}\XS}
\def\Xb{{\sbm{X}}\XS}  \def\xb{{\sbm{x}}\XS}
\def\Yb{{\sbm{Y}}\XS}  \def\yb{{\sbm{y}}\XS}
\def\Zb{{\sbm{Z}}\XS}  \def\zb{{\sbm{z}}\XS}

% ALPHABET CURSIF
% Cursif(majuscules), taille adaptative

\def\Ac{{\ensuremath{\mathcal{A}}}\XS}
\def\Bc{{\ensuremath{\mathcal{B}}}\XS}
\def\Cc{{\ensuremath{\mathcal{C}}}\XS}
\def\Dc{{\ensuremath{\mathcal{D}}}\XS}
\def\Ec{{\ensuremath{\mathcal{E}}}\XS}
\def\Fc{{\ensuremath{\mathcal{F}}}\XS}
\def\Gc{{\ensuremath{\mathcal{G}}}\XS}
\def\Hc{{\ensuremath{\mathcal{H}}}\XS}
\def\Ic{{\ensuremath{\mathcal{I}}}\XS}
\def\Jc{{\ensuremath{\mathcal{J}}}\XS}
\def\Kc{{\ensuremath{\mathcal{K}}}\XS}
\def\Lc{{\ensuremath{\mathcal{L}}}\XS}
\def\Mc{{\ensuremath{\mathcal{M}}}\XS}
\def\Nc{{\ensuremath{\mathcal{N}}}\XS}
\def\Oc{{\ensuremath{\mathcal{O}}}\XS}
\def\Pc{{\ensuremath{\mathcal{P}}}\XS}
\def\Qc{{\ensuremath{\mathcal{Q}}}\XS}
\def\Rc{{\ensuremath{\mathcal{R}}}\XS}
\def\Sc{{\ensuremath{\mathcal{S}}}\XS}
\def\Tc{{\ensuremath{\mathcal{T}}}\XS}
\def\Uc{{\ensuremath{\mathcal{U}}}\XS}
\def\Vc{{\ensuremath{\mathcal{V}}}\XS}
\def\Wc{{\ensuremath{\mathcal{W}}}\XS}
\def\Xc{{\ensuremath{\mathcal{X}}}\XS}
\def\Yc{{\ensuremath{\mathcal{Y}}}\XS}
\def\Zc{{\ensuremath{\mathcal{Z}}}\XS}

% Lettres cursives grasses (majuscules)
%
\def\Acb{{\sbm{\mathcal{A}}}\XS}
\def\Bcb{{\sbm{\mathcal{B}}}\XS}
\def\Ccb{{\sbm{\mathcal{C}}}\XS}
\def\Dcb{{\sbm{\mathcal{D}}}\XS}
\def\Ecb{{\sbm{\mathcal{E}}}\XS}
\def\Fcb{{\sbm{\mathcal{F}}}\XS}
\def\Gcb{{\sbm{\mathcal{G}}}\XS}
\def\Hcb{{\sbm{\mathcal{H}}}\XS}
\def\Icb{{\sbm{\mathcal{I}}}\XS}
\def\Jcb{{\sbm{\mathcal{J}}}\XS}
\def\Kcb{{\sbm{\mathcal{K}}}\XS}
\def\Lcb{{\sbm{\mathcal{L}}}\XS}
\def\Mcb{{\sbm{\mathcal{M}}}\XS}
\def\Ncb{{\sbm{\mathcal{N}}}\XS}
\def\Ocb{{\sbm{\mathcal{O}}}\XS}
\def\Pcb{{\sbm{\mathcal{P}}}\XS}
\def\Qcb{{\sbm{\mathcal{Q}}}\XS}
\def\Rcb{{\sbm{\mathcal{R}}}\XS}
\def\Scb{{\sbm{\mathcal{S}}}\XS}
\def\Tcb{{\sbm{\mathcal{T}}}\XS}
\def\Ucb{{\sbm{\mathcal{U}}}\XS}
\def\Vcb{{\sbm{\mathcal{V}}}\XS}
\def\Wcb{{\sbm{\mathcal{W}}}\XS}
\def\Xcb{{\sbm{\mathcal{X}}}\XS}
\def\Ycb{{\sbm{\mathcal{Y}}}\XS}
\def\Zcb{{\sbm{\mathcal{Z}}}\XS}


% ALPHABET DROIT EN MATHS
% Taille adaptative

\def\AD{{\sdm{A}}\XS}  \def\aD{{\sdm{a}}\XS}
\def\BD{{\sdm{B}}\XS}  \def\bD{{\sdm{b}}\XS}
\def\CD{{\sdm{C}}\XS}  \def\cD{{\sdm{c}}\XS}
\def\DD{{\sdm{D}}\XS}  \def\dD{{\sdm{d}}\XS}
\def\ED{{\sdm{E}}\XS}  \def\eD{{\sdm{e}}\XS}
\def\FD{{\sdm{F}}\XS}  \def\fD{{\sdm{f}}\XS}
\def\GD{{\sdm{G}}\XS}  \def\gD{{\sdm{g}}\XS}
\def\HD{{\sdm{H}}\XS}  \def\hD{{\sdm{h}}\XS}
\def\ID{{\sdm{I}}\XS}  \def\iD{{\sdm{i}}\XS}
\def\JD{{\sdm{J}}\XS}  \def\jD{{\sdm{j}}\XS}
\def\KD{{\sdm{K}}\XS}  \def\kD{{\sdm{k}}\XS}
\def\LD{{\sdm{L}}\XS}  \def\lD{{\sdm{l}}\XS}
\def\MD{{\sdm{M}}\XS}  \def\mD{{\sdm{m}}\XS}
\def\ND{{\sdm{N}}\XS}  \def\nD{{\sdm{n}}\XS}
\def\OD{{\sdm{O}}\XS}  \def\oD{{\sdm{o}}\XS}
\def\PD{{\sdm{P}}\XS}  \def\pD{{\sdm{p}}\XS}
\def\QD{{\sdm{Q}}\XS}  \def\qD{{\sdm{q}}\XS}
\def\RD{{\sdm{R}}\XS}  \def\rD{{\sdm{r}}\XS}
\def\SD{{\sdm{S}}\XS}  \def\sD{{\sdm{s}}\XS}
\def\TD{{\sdm{T}}\XS}  \def\tD{{\sdm{t}}\XS}
\def\UD{{\sdm{U}}\XS}  \def\uD{{\sdm{u}}\XS}
\def\VD{{\sdm{V}}\XS}  \def\vD{{\sdm{D}}\XS}
\def\WD{{\sdm{W}}\XS}  \def\wD{{\sdm{w}}\XS}
\def\XD{{\sdm{X}}\XS}  \def\xD{{\sdm{x}}\XS}
\def\YD{{\sdm{Y}}\XS}  \def\yD{{\sdm{y}}\XS}
\def\ZD{{\sdm{Z}}\XS}  \def\zD{{\sdm{z}}\XS}


% ALPHABET GRAS DROIT
% Permet d'obtenir des caracteres droits directement 
% en mode math ou pas math.
% (Un peu moins utile peut \^eetre)

\def\Av{{\sbv{A}}\XS}  \def\av{{\sbv{a}}\XS}
\def\Bv{{\sbv{B}}\XS}  \def\bv{{\sbv{b}}\XS}
\def\Cv{{\sbv{C}}\XS}  \def\cv{{\sbv{c}}\XS}
\def\Dv{{\sbv{D}}\XS}  \def\dv{{\sbv{d}}\XS}
\def\Ev{{\sbv{E}}\XS}  \def\ev{{\sbv{e}}\XS}
\def\Fv{{\sbv{F}}\XS}  \def\fv{{\sbv{f}}\XS}
\def\Gv{{\sbv{G}}\XS}  \def\gv{{\sbv{g}}\XS}
\def\Hv{{\sbv{H}}\XS}  \def\hv{{\sbv{h}}\XS}
\def\Iv{{\sbv{I}}\XS}  \def\iv{{\sbv{i}}\XS}
\def\Jv{{\sbv{J}}\XS}  \def\jv{{\sbv{j}}\XS}
\def\Kv{{\sbv{K}}\XS}  \def\kv{{\sbv{k}}\XS}
\def\Lv{{\sbv{L}}\XS}  \def\lv{{\sbv{l}}\XS}
\def\Mv{{\sbv{M}}\XS}  \def\mv{{\sbv{m}}\XS}
\def\Nv{{\sbv{N}}\XS}  \def\nv{{\sbv{n}}\XS}
\def\Ov{{\sbv{O}}\XS}  \def\ov{{\sbv{o}}\XS}
\def\Pv{{\sbv{P}}\XS}  \def\pv{{\sbv{p}}\XS}
\def\Qv{{\sbv{Q}}\XS}  \def\qv{{\sbv{q}}\XS}
\def\Rv{{\sbv{R}}\XS}  \def\rv{{\sbv{r}}\XS}
\def\Sv{{\sbv{S}}\XS}  \def\sv{{\sbv{s}}\XS}
\def\Tv{{\sbv{T}}\XS}  \def\tv{{\sbv{t}}\XS}
\def\Uv{{\sbv{U}}\XS}  \def\uv{{\sbv{u}}\XS}
\def\Vv{{\sbv{V}}\XS}  \def\vv{{\sbv{v}}\XS}
\def\Wv{{\sbv{W}}\XS}  \def\wv{{\sbv{w}}\XS}
\def\Xv{{\sbv{X}}\XS}  \def\xv{{\sbv{x}}\XS}
\def\Yv{{\sbv{Y}}\XS}  \def\yv{{\sbv{y}}\XS}
\def\Zv{{\sbv{Z}}\XS}  \def\zv{{\sbv{z}}\XS}


% ALPHABET GREC GRAS 
% Enrichie, completee et modifi\'ee par J.-F. Gio.
% Taille adaptative !

\def\alphab      {{\sbm{\alpha}}\XS}
\def\betab       {{\sbm{\beta}}\XS}
\def\gammab      {{\sbm{\gamma}}\XS}	  \def\Gammab    {{\sbm{\Gamma}}\XS}
\def\deltab      {{\sbm{\delta}}\XS}	  \def\Deltab    {{\sbm{\Delta}}\XS}
\def\epsilonb    {{\sbm{\epsilon}}\XS}
\def\varepsilonb {{\sbm{\varepsilon}}\XS}
\def\etab        {{\sbm{\eta}}\XS}
\def\thetab      {{\sbm{\theta}}\XS}	  \def\Thetab    {{\sbm{\Theta}}\XS}
\def\varthetab   {{\sbm{\vartheta}}\XS}
\def\iotab       {{\sbm{\iota}}\XS}
\def\kappab      {{\sbm{\kappa}}\XS}
\def\lambdab     {{\sbm{\lambda}}\XS}    \def\Lambdab   {{\sbm{\Lambda}}\XS}
\def\mub         {{\sbm{\mu}}\XS}
\def\nub         {{\sbm{\nu}}\XS}
\def\xib         {{\sbm{\xi}}\XS}		  \def\Xib  	  {{\sbm{\Xi}}\XS}
\def\pib         {{\sbm{\pi}}\XS}		  \def\Pib  	  {{\sbm{\Pi}}\XS}
\def\varpib      {{\sbm{\varpi}}\XS}
\def\rhob        {{\sbm{\rho}}\XS}
\def\varrhob     {{\sbm{\varrho}}\XS}
\def\sigmab      {{\sbm{\sigma}}\XS}	  \def\Sigmab    {{\sbm{\Sigma}}\XS}
\def\varsigmab   {{\sbm{\varsigma}}\XS}  \def\Varsigmab {{\sbm{\Varsigma}}\XS}
\def\phib        {{\sbm{\phi}}\XS}  	  \def\Phib 	  {{\sbm{\Phi}}\XS}
\def\varphib     {{\sbm{\varphi}}\XS}
\def\chib        {{\sbm{\chi}}\XS}
\def\psib        {{\sbm{\psi}}\XS}  	  \def\Psib 	  {{\sbm{\Psi}}\XS}
\def\omegab      {{\sbm{\omega}}\XS}	  \def\Omegab    {{\sbm{\Omega}}\XS}
\def\taub        {{\sbm{\tau}}\XS}
\def\upsilonb    {{\sbm{\upsilon}}\XS}   \def\Upsilonb  {{\sbm{\Upsilon}}\XS}
\def\zetab       {{\sbm{\zeta}}\XS}


% CHIFFRES
% Gras, taille adaptative

\def\zerob	 {{\sbv{0}}\XS}
\def\unb		 {{\sbv{1}}\XS}
\def\deuxb	 {{\sbv{2}}\XS}
\def\troisb	 {{\sbv{3}}\XS}
\def\quatreb {{\sbv{4}}\XS}
\def\cinqb	 {{\sbv{5}}\XS}
\def\sixb	 {{\sbv{6}}\XS}
\def\septb	 {{\sbv{7}}\XS}
\def\huitb	 {{\sbv{8}}\XS}
\def\neufb	 {{\sbv{9}}\XS}


% QUELQUES ENSEMBLES
% Taille adaptative

\def\eC{{\ensuremath{\mathbb C}}\XS}
\def\eE{{\ensuremath{\mathbb E}}\XS}
\def\eN{{\ensuremath{\mathbb N}}\XS}
\def\eR{{\ensuremath{\mathbb R}}\XS}
\def\eZ{{\ensuremath{\mathbb Z}}\XS}
\def\eC{{\ensuremath{\mathbb C}}\XS}

